Towards Assurance-Driven Architectural Decomposition of Software Systems

Computer systems are so complex, so they are usually designed and analyzed in terms of layers of abstraction. Complexity is still a challenge facing logical reasoning tools that are used to find software design flaws and implementation bugs. Abstraction is also a common technique for scaling those tools to more complex systems. However, the abstractions used in the design phase of systems are in many cases different from those used for assurance. In this paper we argue that different software quality assurance techniques operate on different aspects of software systems. To facilitate assurance, and for a smooth integration of assurance tools into the Software Development Lifecycle (SDLC), we present a 4-dimensional meta-architecture that separates computational, coordination, and stateful software artifacts early on in the design stage. We enumerate some of the design and assurance challenges that can be addressed by this meta-architecture, and demonstrate it on the high-level design of a simple file system.

==> casestudy.tex <==
%\section{Case Study}
%\label{sec:caseStudy}

\newcommand{\pcalc}{$\pi$-calculus}
\newcommand{\zcalc}{$\zeta$-calculus}
\newcommand{\tnat}{\texttt{nat}}
\newcommand{\valz}{\texttt{z}}
\newcommand{\valsucc}{\texttt{succ}}
\newcommand{\valrec}{\texttt{rec}}
\newcommand{\valwith}{\texttt{with}}
\newcommand{\godel}{G{\"o}del}
\newcommand{\restrict}{\boldsymbol{v}}
\newcommand{\pzero}{\boldsymbol{0}}
\newcommand{\ldef}[1]{{\color{blue} #1}}

\subsection{Example of a Language Design}

\label{sec:lang}

Micro-languages for data, computation and coordination can be designed in lots of different ways, and the interfaces between them can provide different integration capabilities. In this subsection we only give one example of the design of a general purpose programming language based on micro-languages. We illustrate at a high-level how this language can be used to implement the file system component from Sec.~\ref{sec:example}

Fig.~\ref{fig:lang} outlines the syntax of the three micro-languages, with their interaction points \ldef{highlighted in blue}. Fig.~\ref{fig:langCommon} lists the syntactic categories used at the boundaries of the different micro-languages. The micro-languages need to communicate using names or labels. In this design we assume that variable names and field label names are shared among all the micro-languages.

\begin{figure*}[t]
	\begin{subfigure}[c]{0.49\textwidth}
		\centering
		\[
		\begin{array}{lcl}
		x & \in & \{\text{set of computational variables}\} \\
		l & \in & \{\text{set of field labels}\}
		\end{array}
		\]
		\caption{Common syntactic categories}
		\label{fig:langCommon}
	\end{subfigure}
	\hfill
	\begin{subfigure}[c]{0.49\textwidth}
		\centering
		\[
		\begin{array}{lcl}
		O & ::= & [..., l = \ldef{e}, ...] \\
		&  |  & O.[..., l \Leftarrow \ldef{e}, ...] \\
		
		\end{array}
		\]
		\caption{Data micro-language based on a fragment of the \zcalc~\cite{Abadi:1996}.}
		\label{fig:langData}
	\end{subfigure}
	\begin{subfigure}[c]{0.49\textwidth}
		\centering
		\[
		\begin{array}{lcl}
		T & ::= & \tnat ~|~ T_1 \to T_2 \\
		e    & ::= & x	\\
		     &  |  & \valz \\
		     &  |  & \valsucc(e) \\
		     &  |  & \valrec~e\{\valz \hookrightarrow e_0 ~|~ \valsucc(x)~\valwith~y \hookrightarrow e_1\} \\
		     &  |  & \lambda(x : T) e \\
		     &  |  & e_1(e_2) \\
		     &  |  & \ldef{O.l} \\
		\end{array}
		\]
		\caption{Computational micro-language based on \godel's System T~\cite{Harper:2016}}.
		\label{fig:langComp}
	\end{subfigure}
	\hfill
	\begin{subfigure}[c]{0.49\textwidth}
		\centering
		\[
		\begin{array}{lcl}
		c & \in & \{\text{set of channels}\} \\
		n & ::= & c ~|~ \ldef{e} ~|~ \ldef{O} \\
		\pi &  ::=  & \overline{c}n ~|~ c(n) ~|~ [n_1 = n_2] \pi\\
		M & ::= & \pzero ~|~ \pi.P ~|~ M_1 + M_2 \\
		P & ::= & M ~|~ (P_1~|~P_2) ~|~ \restrict c~P \\
		\end{array}
		\]
		\caption{Coordination micro-language based on the \pcalc~\cite{Sangiorgi:2001}.}
		\label{fig:langCoord}
	\end{subfigure}
	\caption{The syntax of a general-purpose programming language based on three micro-languages.}
	\label{fig:lang}
\end{figure*}

\subsubsection{Data Micro-language}

The data micro-language (Fig.~\ref{fig:langData}) is based on a small fragment of the \zcalc~\cite{Abadi:1996}. The syntactic category $O$~defines an object as a set of field labels. Object definition involves assigning a value to each of the field labels. An expression of the form $O.l$~ evaluates to the value bound to the field $l$~of object $O$. Object state mutation atomically updates the value bindings of one or more fields of an object. Please note that we picked a field-only fragment of the \zcalc, leaving out computational methods, because in our design computations belong to the computational micro-language.

In our file system example, a \emph{file} object has three fields: \emph{size}, \emph{creation}, and \emph{permissions}. A simple expression to create an empty file object $f$ with the creation timestamp $t$ and permissions $p$ (where $f$, $t$, and $p$ are variable names) is:
\[
	[size=\valz, creation=t, permissions=p]
\] 

Similarly, the state of $f$ can be atomically updated to change its size to $s * 2$ and its permissions to $q$ using the following expressions:
\[
	f.[size \Leftarrow s *2, permissions \Leftarrow q]
\]

Note that the expressions used to initialize and update individual fields come from the computational micro-language, whose evaluation is guaranteed to terminate. As a result, each expression in the data micro-language is also guaranteed to terminate.

\subsubsection{Computation Micro-language}

The computation micro-language (Fig.~\ref{fig:langComp}) is based on \godel's System T~\cite{Harper:2016}, which is typed $\lambda$-calculus with well-founded recursion (recursive functions are guaranteed to terminate). Built-in types are natural numbers and function types. In addition to variables, $\lambda$-abstractions and applications, \valz~denotes the value zero, and $\valsucc(e)$ denotes the natural number successor of $e$. A recursive function taking an argument $e$ pattern-matches over $e$, with one sub-expression for the \valz~case, and another for the \valsucc~case. The result of a recursive call is bound to variable $y$. Mathematical operators can be implemented as user-defined functions~\cite{Pierce:2002}. The evaluation of System T expressions is guaranteed to terminate~\cite{{Harper:2016}}. 

Mathematical functions used in the file system implementation are to implemented in the computation micro-language. For example, $blockCount$ calculates the number of blocks required to store $n$ bytes, given $blockSize$, and an implementation of $div$, a natural number division operator rounding up. The implementation of $blockCount$ would look like:
\[
	blockCount~n = div~n~blockSize
\]

\subsubsection{Coordination Micro-language}

The coordination micro-language (Fig.~\ref{fig:langCoord}) is an extension of a fragment of the \pcalc~\cite{Sangiorgi:2001}. In the \pcalc, processes communicate by sending messages over channels. In the original \pcalc, the values that can be sent over channels are only channel names. To allow the communication of results of computations and data objects, we allow sending and receiving computational expressions and data objects as well. The syntactic category $n$~is the set of values that can be communicated between processes.

Actions that can be performed by processes are defined by the syntactic category $\pi$. Given a channel $c$ and a value $n$, $\overline{c}n$ is the action send $n$ over $c$, while $c(n)$ is receiving a message from $c$ and binding it to name $n$. An action $\pi$ can be guarded by an equality predicate over two names $n_1$ and $n_2$, i.e., $[n_1 = n_2] \pi$ takes place only if $n_1$ and $n_2$ are names of the same value.

Processes are defined by the two mutually recursive syntactic categories $P$~and $M$. Process $\pzero$~does nothing by definition. An expression $\pi.P$~denotes that process $P$ can proceed only after its guarding action $\pi$ is performed. A sum $M_1 + M_2$ denotes proceeding with only one of the processes $M_1$ and $M_2$, based on which of them can perform its guarding action. 

Parallel composition of two processes $P_1$ and $P_2$ is denoted by $P_1~|~P_2$. The two processes can communicate using shared names. An expression $\restrict c~P$ restricts the scope of channel name $c$ to the process expression $P$.

Please note that the fragment of the \pcalc~we are using here does not include the process replication operator, which in standard \pcalc~allows for the recursive definition of processes. Recursion (using replication or other approaches) is what makes standard \pcalc~Turing-complete~\cite{Gorrieri:2017}. Our coordination micro-language is thus not Turing-complete. 

Assuming we have a $write$ communication channel between a user-mode process and the file system, and a $reserve$ channel between the file system and the storage system. When the file system receives a number of bytes to be written over the $write$ channel, it sends the number of blocks to be reserved for the bytes to be written to the storage manager over the $reserve$ channel. Since the number of blocks is to be calculated, the computational expression for that calculation can be passed over the channel directly as follows:
\[
	write(n).\overline{reserve}(blockCount~n)
\]
%\subsection{File System Read/Write}

%\todo{read operation}

%\todo{write operation}


==> fallacies.tex <==
\section{Misconceptions}
\label{sec:fallacies}

In this section we discuss some of the points usually made when arguing for Turing-completeness in programming language design, and argue that those points might not be strong enough.

\subsection{Reactive Systems and Turing-Completeness}
\label{sec:reactive}

Probably the most commonly used argument made for Turing-completeness in general-purpose programming languages is addressing non-termination in reactive systems. Similar to our motivating example in Sec.~\ref{sec:example}, many systems involve continuously waiting indefinitely for events and processing them as they arrive. This is how web servers, Graphical User Interfaces (GUIs), and messaging applications on smart phones interact with their users. However, it is important to note that waiting for events is not computing. Sending and receiving messages are not computing either. In our file system example, computations are all finite. Those computations might be triggered by specific events or messages, but they do not participate in the coordination protocol between processes.

As a matter of fact, computations are required to be finite. Imagine any of the computations in Fig.~\ref{fig:example} falling into an infinite loop due to a coding bug. That would put the file system, and effectively the whole operating system, in an unresponsive state. In his seminal book The Art of Computer Programming, Donald Knuth characterizes the notion of an algorithm in terms of five attributes, the first of which is finiteness. In his definition of algorithms, Knuth explicitly states that "an algorithm must always terminate after a finite set of steps"~\cite{Knuth:1997}.

But reactive systems still need those indefinite event loops. Harel and Pnueli characterize a reactive system as a system that "..., in general, does not compute or perform a function, but is supposed to maintain a certain ongoing relationship, so to speak, with its environment"~\cite{Harel:1985}. To support the development of reactive systems, we do not really need more computational expressibility. Instead, we need different formalisms where communication, coordination and interaction are first-class constructs. Process calculi exactly serve that purpose. 

%A more suitable approach to address this problem is process calculi rather than computational languages. 
A process calculus is a formal language for defining systems of communicating processes. Examples include Communicating Sequential Processes (CSP)~\cite{Hoare:1978}, Calculus of Communicating Systems (CCS)~\cite{Milner:1980}, Algebra of Communicating Processes (ACP)~\cite{Bergstra:1989}, and the $\pi$-calculus~\cite{Milner:1999}. One benefit of defining process communication behavior in a language different from that used to define computations is avoiding any unintentional interference between the two. This sort of separation of concerns at the meta-level leads towards cleaner designs of programming languages, and also safer software systems.
 
\subsection{Computability and Turing Completeness}

Another common argument for Turing-complete languages is expressibility of algorithms. It is known that primitive recursion is not enough to express some mathematical functions, that can be only expressed using general recursion~\cite{Boolos:2007}. Ackermann function is usually cited as the simplest example of such functions. It is true that formalisms and languages come with different expressive powers, and that (according to the Church-Turing thesis) Turing-complete languages are at the top of that expressiveness pyramid. However, giving up Turing-completeness does not necessarily mean resolving to primitive recursion.

Over the last few decades several Turing-incomplete languages with support for general recursion have been designed. Examples are particularly found in interactive theorem provers based on constructive logic. Gallina~\cite{Huet:1992}, the functional language used in the Coq~\cite{Bertot:2010} interactive theorem prover is one such language. Another more recent example is the language used in the Lean theorem prover~\cite{deMoura:2015} (language is also called Lean). A definition of Ackermann function in Lean is included in one of the Lean manuals~\cite{Avigad:2020}.

\subsection{Processes Calculi and Turing Completeness} 

As mentioned in Sec.~\ref{sec:reactive}, process calculi can be used instead of computational languages to define coordination (communication and synchronization) aspects of systems. Many process calculi have been proven to be Turing-complete though, which might appear like defeating the purpose of using them in the first place. For example, it has been proven that the $\pi$-calculus is as computationally expressive as the $\lambda$-calculus~\cite{Milner:1992}. An arbitrary Systems modeled in $\pi$-calculus can be transformed to CCS~\cite{Banach:1998}, which is effectively a proof that CCS is also Turing-complete. The fact that many process calculi allow for a countably infinite number of constants (processes) and actions (messages), together with message replication, enables encoding mathematical objects (e.g., natural numbers) in those calculi, and allows for applying function-like operations to them.

Moreover, some process calculi with finite constants and actions have been proven to be Turing-complete. For example, the CCS(25,12) calculus (with 25 constants and 12 actions) is Turing-complete~\cite{Gorrieri:2017}. However, in that same paper~\cite{Gorrieri:2017} the author argues that Turing-completeness is probably not the right metric to measure the expressive power of process calculi, or formalisms for defining concurrent systems in general. In addition, the author also gave an example of a concurrency problem (Last Man Standing) that can not be expressed in Turing-complete languages. This further highlights the fact that computation and coordination are fundamentally different, and that their languages should be defined separately~\cite{Gelernter:1992}.


\subsection{Small Core and Syntactic Sugar}

The design of programming languages involves many challenges, one of which is the definition of robust semantics of each language construct. Because of the numerous different ways in which language constructs can interfere with each other, it has been a common practice to design a language with a relatively small core, and then design more features in the form of "syntactic sugar" on top. This practice has been justified by many problems of widely-used languages with relatively big cores. Examples include the numerous cases of undefined behavior of constructs of C and C++, and type system unsoundness of Java and Scala~\cite{Amin:2016}.

As a language tries to be ubiquitous, the small core design philosophy becomes a limitation though. For example, for an inherently sequential language to support concurrency, an asynchronous message from one process to another can be \emph{emulated} as a construct available in the small core (e.g., a procedure call). Similarly, for a pure functional language to support effectful actions (e.g., I/O operations or mutable state), those actions are typically wrapped in Monads. This is not necessarily a drawback of the small core principle, but rather a disadvantage of having a \emph{single} core.

In Sec.~\ref{sec:multicore} we argue that for a language to support computation, coordination, and stateful objects, it is both safer and more efficient to design a language with multiple small cores instead of one. Because each of the cores models a different aspect of software functionality, it will be more focused on that aspect only, and it will have a higher degree of freedom to include constructs and formalisms that might not be relevant to the other cores. 

==> future.tex <==
\section{Future Directions}
\label{sec:future}

Reaching the right balance between providing highly expressive language features while at the same time restricting those features to decisively stop a programmer from "shooting himself in the foot" will always be an area of many research and design challenges. Because of the theoretical aspects involved in the crossroads of Computability theory, Complexity theory, program semantics and type theory, addressing those challenges can be considered both an art and a science. Some of the research questions involved are briefly outlined in the following subsections.

\subsection{Reactive Systems}

Reactive systems are, by definition, looping for ever. The operating system of any computer of any form factor has to be up all the time, waiting for user or system events to handle. A web server is similarly up all the time, waiting for web requests to the server. Embedded systems used to control TV sets, vehicle, airplanes and nuclear power reactors vary in criticality, but they all share the property of continuously interacting with their environment rather than simply running an algorithm on some inputs, resulting on some outputs and then halting. Obviously a terminating language by itself is not enough to meet those requirements, but at the same solutions other than Turing-Completeness are available, and probably better suited, for the problem.

It is important to realize that event handling has nothing computational to it. A program waiting for an event out of a set of events to happen, and takes a simple action based on which event took place, and keep repeating that behavior for ever, consequently has nothing computational to it as long as those simple actions do not compute anything. Finite-state automata have been used to model and implement such systems for a long time.

Now it is the actions taken by an automaton that can be computational in nature. For example, the braking system of a car might need to make some calculations whenever the driver hits the brakes. The algorithm for those calculations is implemented in a programming language, and obviously the computation has to terminate, otherwise the braking system will get stuck, and the action expected from hitting the brakes will never take place. It is important to note that, by design, the automaton has to continuously respond to events (essentially looping forever), while the computational procedure, again by design, has to not just terminate, but also terminate in a timely manner.

Given the distinct characteristics and requirements of the automata responsible for the reactive behavior and the programs responsible for the computational aspects of a system, having distinct languages, based on different theoretical foundations, for each of those orthogonal aspects of systems development might be the way to go.

Several process calculi (CCS, CSP, pi-calculus, etc...) have been developed to model parallel, concurrent, distributed, reactive and mobile systems. Some of those calculi are even Turing-Complete, which again might be an overkill given the fact that they are not addressing computation in the first place. Lambda calculus on the other hand is an underlying theory of computation. Restricted forms of lambda calculus, limiting recursion, can effectively model terminating, and thus can be used as a foundation for computational languages. Similarly, process calculi can be used as the theoretical foundation of coordination languages, modeling only communication, coordination and interaction between coordination modules, and also for coordination modules to invoke computational modules as needed.

One more advantage for separating computations from coordination is that verifying each of them separately will be significantly easier. Algorithms, and their corresponding computational procedures, are sequential by nature. Correctness properties of computational procedures simply involve input/output relationships, so they can be simply specified in terms of preconditions and postconditions. In the absence of concurrency, race conditions and the possibility of deadlocks, axiomatic frameworks and theorem provers are best suited for verifying the correctness of sequential computational procedures.

On the other hand coordination modules involve several parties communicating together, so they are concurrent by nature. Model checkers have been used for a few decades to verify concurrent hardware and software systems. The biggest problem facing model checking is scalability with respect to the state space of the model being checked. Taking the computational aspects completely out of the picture and simply abstracting them in terms of preconditions and postconditions significantly simplifies the state space of a system, automatically scaling up the power of existing model checkers to more complex systems.

\subsection{Looping/Recursion Constructs}

Since the early days of high-level languages, looping and recursion have been essential ingredients of pragmatic languages. LISP, the grandparent of all functional languages, adopted recursion directly from the lambda calculus, while FORTRAN, the pioneering imperative language at the time, introduced imperative looping constructs. In both cases nothing prevented a program from iterating (recursing or looping) forever, and this continued to be the case for the vast majority of programming languages since then.
Terminating languages on the other hand restrict recursion and/or iteration. Gallina for example imposes a simple restriction on recursive calls: at least one of the parameters of the recursive call has to decrease. Since data types in Gallina are all Algebraic Data Types, it is easy to check statically against that rule. It is known though that this rule is sometimes too restrictive, rejecting valid problems because they do not literally follow the decreasing parameter rule, or because the decreasing property is not obvious enough for the compiler. This kind of problem needs to be addressed by designing more robust looping and recursion constructs that are both highly expressive and guaranteed to terminate.

\subsection{Recursive Data Structures}

What happens if a linked list traversal procedure is known to terminate, but the list passed to the procedure happens to have a cycle? Obviously the otherwise terminating procedure will keep looping forever, simply because in many programming languages nothing prevents a linked list to violate its semantic contract and end up having a cycle. This example demonstrates the importance of designing both control and data constructs together if termination is required.

Algebraic Data Types (ADTs) in the absence of mutable references is one way of solving that problem. A list or a tree ADT in Gallina for example is guaranteed to be both finite and acyclic, because each node is freshly created by a constructor and both structures are immutable. This might be enough for a language primarily used for proving the correctness of simple algorithms, but for a general purpose, high performance language will probably need both references and mutation constructs.

Designing data definition constructs that would specify both safe and efficient data structures has another potential set of research questions associated with it. For example object identity guarantees and tracking, safe state transitions for objects with respect to object invariants, hierarchical objects, object ownership and garbage collection are all research areas that are directly involved in addressing those research questions.



==> macros_spl.tex <==
%% Software Product Line (SPL) macros
\DeclareMathOperator{\Prop}{Prop}
\DeclareMathOperator{\Conf}{Conf}

\newcommand{\pc}[1]     {pc_{#1}}
\newcommand{\spl}       {\mathcal{L}}
\newcommand{\feat}[1]{\code{#1}} %for features
\newcommand{\featset}{F}
\newcommand{\featmodel}{\Phi}
\newcommand{\domainmodel}{D}
\newcommand{\pcmap}{\phi}
\newcommand{\conf}{\rho}
\newcommand{\PC}[1]{\texttt{#1}}
\newcommand{\indexconf}[2]{#1|_{#2}}
\newcommand{\indexProd}[2]{#1|_{#2}}
\newcommand{\restrictconf}[2]{#1||_{#2}}

\newcommand{\F}               {F}
\newcommand{\FM}              {\Phi}

% keywords and concepts
\newcommand{\cppifdef}{\texttt{\#ifdef}}
\newcommand{\cppendif}{\texttt{\#endif}}

\newcommand{\souffle}{\idx{Souffl\'{e}}}
